A short term credibility index for central banks under inflation targeting: an application to Brazil

This paper uses predictive densities obtained via mixed causal-noncausal autoregressive models to evaluate the statistical sustainability of Brazilian inflation targeting system with the tolerance bounds. The probabilities give an indication of the short-term credibility of the targeting system without requiring modelling people's beliefs. We employ receiver operating characteristic curves to determine the optimal probability threshold from which the bank is predicted to be credible. We also investigate the added value of including experts predictions of key macroeconomic variables.

==> 7-Discussion.tex <==
\section{Discussion}

After having estimated the MAR($1,1)$ model for the Brazilian year to year
annual inflation rate series $\pi_{t}=(1-L^{12})\ln P_{t},$ it emerged that we still observed in the correlogram of the residuals $\hat{\varepsilon}_{t}$ in $(1-\hat{\phi}_{1}L)(1-\hat{\varphi}_{1}L^{-1})\pi_{t}=\hat{\varepsilon}_{t}$ a dependency at displacement 12. This feature emphasizes the presence of a stochastic seasonal component similar to what we can observe in ARIMA models that are extended to SARIMA models to account for that seasonal pattern. It would be probably misleading in small samples to estimate an autoregressive pseudo causal model up to lag orders $p=12$ or 13. First, none of the information criteria would go so far given that lags from 3 to 11 are probably non significantly different from zero. Second, in the event that we would get that large lag order using e.g. BIC, the combination of all possible MAR($r,s$) within $p=12$ or 13 would make the identification of MAR models doubtful. \\

Consequently, we propose a new modeling that takes into account potential seasonality. It is an extension of standard MAR(\textit{r},\textit{s}) model augmented with seasonal components, denoted as SMAR(\textit{r},\textit{s})(\textit{R},\textit{S}). The model is constructed as follows, 
\begin{equation}
    (1-\phi^* L^{R})(1-\psi^* L^{-S})\Phi(L)\Psi(L^{-1})y_{t}=\varepsilon_{t},
\end{equation}
where $\Phi(L)\Psi(L^{-1})y_{t}$ has the standard structure of an MAR(\textit{r,s}). The SMAR introduces a multiplicative seasonal dependency (leads and/or lags) at displacements \textit{R} and \textit{S} for the backward- and forward-looking seasonality. For simplicity, we assume that each of the two seasonal components are of order 1 maximum. That is, \textit{R} and \textit{S} are integers indicating the displacements of the seasonality in each direction.\footnote{We could for instance think of a generalisation of the model with \textit{R} and \textit{S} being vectors indicating various displacements of seasonality.} We further assume, analogously to standard MAR models, that the roots of all lag polynomials lie outside the unit circle. That is, $\Phi (z)=0,$ $\Phi ^{\ast }(z)=0,$ $\Psi (z)=0$ and $\Psi ^{\ast }(z)=0$ for $|z|>1.$ \\

The approach we propose to identify and estimate SMAR(\textit{r},\textit{s})(\textit{R},\textit{S}) models is as follows,
\begin{enumerate}

\item We first identify and estimate the non seasonal MAR($r,s$) model by AMLE starting with
the pseudo causal model in which $p$ is determined by BIC. Then, the MAR(\textit{r,s}) such that $r+s=p$ is identified as the model with the highest likelihood value.

\item Then, we investigate potential left over seasonal patterns in the residuals sequence of the estimated MAR(\textit{r,s}). 

\item In case some seasonality has been detected at distinct displacements (which we limit to 2 for simplicity here, say $D_1$ and potentially $D_2$), we estimate by AMLE the 2 following SMAR models,
\begin{equation*}
    \begin{split}
        (1-\phi^* L^{D_1})(1-\psi^* L^{-D_2})\Phi(L)\Psi(L^{-1})y_{t}&=\varepsilon_{t}\\
        (1-\phi^* L^{D_2})(1-\psi^* L^{-D_1})\Phi(L)\Psi(L^{-1})y_{t}&=\varepsilon_{t},
    \end{split}
\end{equation*}
where $\Phi(L)$ and $\Psi(L^{-1})$ are of order \textit{r} and \textit{s} as estimated in the first step. We favour the model with the highest likelihood value. The estimation of the model is done analogously to regular MARs, that is by linearizing the parameters we estimate under nonlinear constraints by Student's $t$ AMLE. \\

\item Forecasting with this model is far from trivial and we leave it for further research.

\end{enumerate}


In the case investigated in this paper, when estimating the pseudo lag order \textit{p} at step 1, which we identify as being 2, it can be misleading as the seasonal component is not seen by the sequence of information criteria which consider all lags up until $p^{\ast }=0...15$. With that $p=2$, we have identified the best fitting model on monthly year-on-year inflation rate to be an MAR(1,1). We then detected seasonality in the residuals of the MAR(1,1) at displacement 12. We then compared SMAR(1,1)(12,0) and SMAR(1,1)(0,12) and favoured the latter given the likelihood values. The estimated model is the following,
\begin{equation}
    (1+0.30L^{-12})(1-0.59L)(1-0.96L^{-1})\pi_{t}=\varepsilon_{t},
\end{equation}
with $\varepsilon_t$ a Student`s-\textit{t} distribution with 3.99 degrees of freedom. The MAR coefficients and the degrees of freedom are thus almost the same as for the standard MAR(1,1) estimated previously. This implies that monthly year-on-year inflation rates have a forward looking seasonality component additionally to the mixed causal-noncausal dynamics implied by the MAR model. We find no remaining seasonality or autocorrelation left in the residuals of the SMAR model. Expanding the model in its additive form yields the following, 
\begin{equation}
    \begin{split}
        \pi_t&=\frac{\phi}{1+\phi\psi}\pi_{t-1}+\frac{\psi}{1+\phi\psi}\pi_{t+1}-\frac{\phi\psi^*}{1+\phi\psi}\pi_{t+11}+ \\
        & \hspace{+2cm}+\frac{\psi^*+\phi\psi\psi^*}{1+\phi\psi}\pi_{t+12}-\frac{\psi\psi^*}{1+\phi\psi}\pi_{t+13}+\frac{1}{1+\phi\psi}\varepsilon_t\\
        \\
        \pi_t&=0.38\pi_{t-1}+0.61\pi_{t+1}+0.11\pi_{t+11}-0.30\pi_{t+12}+0.18\pi_{t+13}+\varepsilon^*_t
    \end{split}
\end{equation}

{\color{red} Besides the difficulty to forecast with such model, another rising issue is the loss of the last 13 data points, which are the points of interest from which the forecasts should be performed. Alternatives that we suggest are for instance the inclusion of the seasonality in causal time, which, within the SMAR framework would be straightforward, even for forecasting. The use of the seasonality in causal time could also allow for 1-year ahead one-step forecasts of inflation, which are often of interest, as shown by the various credibility indices described in Section \ref{bra-sec:Credibility}. While we know model \eqref{bra-eq:MAR_infl} is not optimal, we leave the introduction of the remaining noncausal stochastic seasonality within MAR framework for forecasting for further research. In line with the NKPC model \eqref{eq:NKPC}, the \textit{i.i.d.} assumption of the error term could also be violated from the inherent dynamics of the omitted variables $x_t$. The seasonality could then also be accounted for with the inclusion of exogenous seasonal variables.}
